Ly$\alpha$ emission as a sensitive probe of feedback-regulated LyC escape from dwarf galaxies

Ly$\alpha$ emission is an exceptionally informative tracer of the life cycle of evolving galaxies and the escape of ionising photons. However, theoretical studies of Ly$\alpha$ emission are often limited by insufficient numerical resolution, incomplete sets of physical models, and poor line-of-sight (LOS) statistics. To overcome such limitations, we utilize here the novel PANDORA suite of high-resolution dwarf galaxy simulations that include a comprehensive set of state-of-the-art physical models for ionizing radiation, magnetic fields, supernova feedback and cosmic rays. We post-process the simulations with the radiative transfer code \textsc{RASCAS} to generate synthetic observations and compare to observed properties of Ly$\alpha$ emitters. Our simulated Ly$\alpha$ haloes are more extended than the spatial region from which the intrinsic emission emanates and our spatially resolved maps of spectral parameters of the Ly$\alpha$ emission are very sensitive to the underlying spatial distribution and kinematics of neutral hydrogen. Ly$\alpha$ and LyC emission display strongly varying signatures along different LOS depending on how each LOS intersects low-density channels generated by stellar feedback. Comparing galaxies simulated with different physics, we find the Ly$\alpha$ signatures to exhibit systematic offsets determined by the different levels of feedback strength and the clumpiness of the neutral gas. Despite this variance, and regardless of the different physics included in each model, we find universal correlations between Ly$\alpha$ observables and LyC escape fraction, demonstrating a robust connection between Ly$\alpha$ and LyC emission. Ly$\alpha$ observations from a large sample of dwarf galaxies should thus give strong constraints on their stellar feedback-regulated LyC escape and confirm their important role for the reionization of the Universe.

==> bg_liter.tex <==
\section{Observations of high-z universe}

\subsection{\citet{Witstok21a, Witstok21b}}

Sherwood with on-the-fly self-shielding


\section{LAE}

\subsection{X-Shooter \citep{Matthee21} }

\subsection{\citet{Gnedin08}}


